ORION: A Holistic End-to-End Autonomous Driving Framework by Vision-Language Instructed Action Generation

End-to-end (E2E) autonomous driving methods still struggle to make correct decisions in interactive closed-loop evaluation due to limited causal reasoning capability. Current methods attempt to leverage the powerful understanding and reasoning abilities of Vision-Language Models (VLMs) to resolve this dilemma. However, the problem is still open that few VLMs for E2E methods perform well in the closed-loop evaluation due to the gap between the semantic reasoning space and the purely numerical trajectory output in the action space. To tackle this issue, we propose ORION, a holistic E2E autonomous driving framework by vision-language instructed action generation. ORION uniquely combines a QT-Former to aggregate long-term history context, a Large Language Model (LLM) for driving scenario reasoning, and a generative planner for precision trajectory prediction. ORION further aligns the reasoning space and the action space to implement a unified E2E optimization for both visual question-answering (VQA) and planning tasks. Our method achieves an impressive closed-loop performance of 77.74 Driving Score (DS) and 54.62% Success Rate (SR) on the challenge Bench2Drive datasets, which outperforms state-of-the-art (SOTA) methods by a large margin of 14.28 DS and 19.61% SR.

==> table/main_table_and_multi_ability.tex <==

\begin{table*}[tp!]
\centering
\caption{Closed-loop, Open-loop and Multi-Ability Results of E2E-AD Methods in Bench2Drive under base set. C/L refers to camera/LiDAR. Avg.L2 is averaged over the predictions in 2 seconds under 2Hz, similar to UniAD. * denote expert feature distillation. Ref: Reference, Con: Condition, Mod: modality, NC: navigation command, TP: target point, DS: Driving Score, SR: Success Rate, Eff: Efficiency, Com: Comfortness, M: Merging, O: Overtaking, EB: Emergency Brake, GW: Give Way, TS: Traffic Sign.
\label{tab: main result and multi ability}}
% \resizebox{1.0\textwidth}{!}{\begin{tabular}{l| c | c c c c}
\footnotesize
\setlength\tabcolsep{0.45 mm} %列
\begin{tabular}{l c c c  >{\columncolor{gray!10}}c >{\columncolor{gray!10}}c c c   c  ccccc >{\columncolor{gray!10}}c}
\toprule
\multirow{2.2}{*}{Method} & \multirow{2.2}{*}{Ref} &\multirow{2.2}{*}{Con} &\multirow{2.2}{*}{Mod}  & \multicolumn{4}{c}{Closed-loop}  & \color{gray}Open-loop  & \multicolumn{6}{c}{Ability (\%) $\uparrow$} \\ 
    \cmidrule(lr){5-8}  \cmidrule(lr){9-9} \cmidrule(lr){10-15} & & &  &  DS$\uparrow$   & SR(\%)$\uparrow$ & Eff.$\uparrow$  & Com.$\uparrow$ &  \color{gray} Avg.L2 (m) $\downarrow$ & {M}& {O} & {EB} & {GW} & TS& Mean  \\ \midrule

TCP*~\cite{wu2022trajectoryguided}& NeurIPS 22 & TP & C   &  40.70     & 15.00  & 54.26 & 47.80  & \color{gray}1.70  & 16.18        & 20.00           & 20.00        &  10.00         & 6.99     & 14.63     \\
TCP-ctrl* &NeurIPS 22  & TP    & C   &  30.47    & 7.27  & 55.97 & 51.51 & \color{gray}-  & 10.29        & 4.44           & 10.00        &  10.00          & 6.45     & 8.23        \\
TCP-traj* & NeurIPS 22& TP & C   &  59.90     & 30.00 & 76.54 & 18.08    & \color{gray}1.70   & 8.89       & 24.29           & 51.67       &  40.00        & 46.28    & 34.22     \\
TCP-traj w/o distillation & NeurIPS 22  & TP   & C    &  49.30     & 20.45  & 78.78 & 22.96  & \color{gray}1.96  & 17.14       & 6.67           & 40.00       &  50.00    & 28.72    & 28.51     \\
ThinkTwice*~\cite{jia2023thinktwice}  & CVPR 23 & TP & C   & 62.44     & 31.23  & 69.33 & 16.22   & \color{gray}0.95  & 27.38       &  18.42          & 35.82       &  50.00        & 54.23    & 37.17      \\
DriveAdapter*~\cite{jia2023driveadapter} &ICCV 23 & TP & C\&L   &  64.22   & 33.08 & 70.22 & 16.01    & \color{gray}1.01 & 28.82       &26.38           & 48.76      &  \textbf{50.00}         & 56.43   & 42.08        \\  

\midrule

AD-MLP~\cite{zhai2023ADMLP} & arXiv 23 &  NC &C    & 18.05     &  0.00  & 48.45 &   22.63  & \color{gray}3.64 & 0.00        & 0.00           & 0.00        & 0.00         &  4.35    & 0.87      \\
UniAD-Tiny~\cite{hu2023planning} & CVPR 23 & NC & C   & 40.73    & 13.18 & 123.92 & 47.04  &  \color{gray}0.80  & 8.89        & 9.33           & 20.00       & 20.00        & 15.43    & 14.73         \\
UniAD-Base~\cite{hu2023planning} & CVPR 23 & NC  & C  & 45.81     & 16.36 & 129.21 & 43.58  & \color{gray}0.73  & 14.10       & 17.78          & 21.67       &  10.00       & 14.21    & 15.55      \\

% UniAD-Base$^\dagger$~\cite{hu2023planning} & CVPR 23 & NC  & C  & 34.90     & 12.73 & 144.95 & 42.36  & \color{gray}0.73 & 13.56       & 13.64         & 23.08      &  10.00      & 17.86  & 15.63     \\

VAD~\cite{jiang2023vad}& ICCV 23 & NC & C  &42.35     & 15.00 & 157.94 & 46.01  &  \color{gray}0.91  & 8.11       & 24.44         & 18.64       &  20.00       & 19.15    & 18.07     \\

% VAD~\cite{jiang2023vad}$^\dagger$ & ICCV 23 & NC & C  &39.51    & 15.45 & 162.38 & 44.71  &  \color{gray}0.91  & 10.14       & 20.00         & 25.00      &  10.00      & 14.74  & 15.98    \\ 
GenAD~\cite{zheng2024genad} & ECCV 24 & NC &C & 44.81 & 15.90 &  -& - &\color{gray}- &- &- &- &- &- &-\\
MomAD\cite{song2025don} & CVPR 25 & NC & C & 44.54	&16.71&	170.21&	48.63& \color{gray}0.87&- &- &- &- &- &-\\
DriveTransformer-Large~\cite{jiadrivetransformer} & ICLR 25 & NC   & C & 63.46     & 35.01 & 100.64 & 20.78  &  \color{gray}\textbf{0.62} & 17.57 & 35.00 & 48.36 & 40.00 &52.10 &38.60 \\ 

\midrule
\rowcolor[RGB]{230, 242, 255} ORION (\textbf{Ours})  & - & NC & C & \textbf{77.74}\dplus{+14.28}  & \textbf{54.62}\dplus{+19.61} & 151.48& 17.38 & \color{gray}0.68  & 25.00 & \textbf{71.11} &\textbf{78.33}  &30.00 &\textbf{69.15} &\textbf{54.72}\dplus{+16.12} \\

\bottomrule
\end{tabular}
\end{table*}
% \ddplus{+14.28} \ddplus{+19.61}
